ScienceBuddy: Recursive-in-Recursive Self-Improvement for Interactive Scientific Agents

We introduce and release ScienceBuddy, an interactive scientific research workspace that brings continually improving scientific agents into researchers' everyday workflows. ScienceBuddy supports researchers in carrying out scientific tasks while transforming their requests, feedback, and execution evidence into tasks and evaluation rubrics for continual learning. At its core is recursive-in-recursive self-improvement, a paradigm that couples harness evolution with model reinforcement learning: the inner recursion improves the harness with the model fixed, while the outer recursion trains the model under the improved harness. Harness evolution shapes training experience, and model learning creates new opportunities for harness adaptation. We present case studies of researcher interaction, harness refinement, and model learning, with the benchmark cases spanning four scientific task families. By releasing ScienceBuddy as a research product, we make this paradigm available to the scientific community and take a step toward discovery intelligence: scientific AI that advances through sustained collaboration with researchers and evolves alongside the research it supports. Website: http://science-buddy.io

==> frontmatter-layout.tex <==
% Paper-local title-page layout; phai.cls retains the original defaults.
% The three-line title and abstract text are unchanged.
\makeatletter
\renewcommand\phai@titlefont{\linespread{1}\fontsize{19}{22}\selectfont}
\patchcmd{\phai@titleblock}{\vspace{6mm}}{\vspace{1mm}}{}{}
\patchcmd{\phai@titleblock}{\vspace{6mm}}{\vspace{1mm}}{}{}
% Give the author block breathing room below the title divider.
\patchcmd{\phai@titleblock}{\vspace{5.5mm}}{\vspace{3mm}}{}{}
% Balance the product-link row between contribution notes and the abstract.
\patchcmd{\maketitle}{\vspace{6mm}}{\vspace{-6.5mm}}{}{}

\patchcmd{\phai@titleblock}{\vspace{2.2mm}}{\vspace{0.8mm}}{}{}
% Compact author and contribution lines preserve room for the page-one teaser.
\patchcmd{\phai@titleblock}{\sffamily\bfseries\fontsize{11.5}{15}}{\rmfamily\mdseries\linespread{1}\fontsize{9.5}{11.5}}{}{}
\patchcmd{\phai@titleblock}{\vspace{1.4mm}}{\vspace{2.5mm}}{}{}
\patchcmd{\phai@titleblock}{\fontsize{9}{12}}{\linespread{1}\fontsize{8}{9.5}}{}{}

% A full-width, compact card with the original type size and color scheme.
\renewenvironment{abstract}{%
  \begin{tcolorbox}[enhanced, colback=white, colframe=phaideep,
    boxrule=0.5pt, arc=2mm, outer arc=2mm,
    left=5mm, right=5mm, top=1.5mm, bottom=1.5mm,
    width=\linewidth, grow to left by=0pt, grow to right by=0pt,
    before skip=-1.5mm, after skip=4mm]
  \setlength{\parskip}{0pt}%
  {\centering\sffamily\bfseries\fontsize{11}{13}\selectfont\color{phaiaccent}Abstract\par}
  \vspace{1mm}
  \linespread{1}\fontsize{9.5}{11}\selectfont\color{phaiink}\ignorespaces}
 {\ifdefempty{\phai@ledger}{}{\vspace{1mm}\phai@ledger}%
  \end{tcolorbox}}

% First-page masthead: retain PhAI Labs at left and use the official product logo at right.
\fancypagestyle{phaifirst}{%
  \fancyhf{}\renewcommand\headrulewidth{0pt}\renewcommand\footrulewidth{0pt}%
  \fancyhead[L]{\phai@dropped{\phailockup[\phai@logosize]}}%
  \fancyhead[R]{\phai@dropped{\raisebox{-0.18\height}{\includegraphics[height=13mm]{figures/sciencebuddy-official-lockup.pdf}}}}%
  \fancyfoot[C]{\sffamily\fontsize{8.6}{11}\selectfont\color{phaifaint}\thepage}}
\makeatother

% Compact caption applied only to the title-page overview.
\DeclareCaptionFont{overviewcaption}{\linespread{1}\fontsize{8.3}{10}\selectfont}

% Keep only the caption's normal gap below the title-page graphic.
\newcommand{\frontoverview}[2]{%
  \begingroup\centering
  #1\par
  \captionof{figure}{#2}%
  \endgroup}

